Many-body cavity quantum electrodynamics with driven inhomogeneous emitters

Quantum emitters coupled to optical resonators are quintessential systems for exploring fundamental phenomena in cavity quantum electrodynamics (cQED) and are commonly used in quantum devices acting as qubits, memories and transducers. Many previous experimental cQED studies have focused on regimes in which a small number of identical emitters interact with a weak external drive, such that the system can be described with simple, effective models. However, the dynamics of a disordered, many-body quantum system subject to a strong drive have not been fully explored, despite its importance and potential in quantum applications. Here we study how a large, inhomogeneously broadened ensemble of solid-state emitters coupled with high cooperativity to a nanophotonic resonator behaves under strong excitation. We discover a sharp, collectively induced transparency (CIT) in the cavity reflection spectrum, resulting from quantum interference and collective response induced by the interplay between driven inhomogeneous emitters and cavity photons. Furthermore, coherent excitation within the CIT window leads to highly nonlinear optical emission, spanning from fast superradiance to slow subradiance. These phenomena in the many-body cQED regime enable new mechanisms for achieving slow light and frequency referencing, pave a way towards solid-state superradiant lasers and inform the development of ensemble-based quantum interconnects.

==> latexmkrc <==
%auto-ignore
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
